Transporting Higher-Order Quadrature Rules: Quasi-Monte Carlo Points and Sparse Grids for Mixture Distributions

Integration against, and hence sampling from, high-dimensional probability distributions is of essential importance in many application areas and has been an active research area for decades. One approach that has drawn increasing attention in recent years has been the generation of samples from a target distribution $\mathbb{P}_{\mathrm{tar}}$ using transport maps: if $\mathbb{P}_{\mathrm{tar}} = T_\# \mathbb{P}_{\mathrm{ref}}$ is the pushforward of an easily-sampled probability distribution $\mathbb{P}_{\mathrm{ref}}$ under the transport map $T$, then the application of $T$ to $\mathbb{P}_{\mathrm{ref}}$-distributed samples yields $\mathbb{P}_{\mathrm{tar}}$-distributed samples. This paper proposes the application of transport maps not just to random samples, but also to quasi-Monte Carlo points, higher-order nets, and sparse grids in order for the transformed samples to inherit the original convergence rates that are often better than $N^{-1/2}$, $N$ being the number of samples/quadrature nodes. Our main result is the derivation of an explicit transport map for the case that $\mathbb{P}_{\mathrm{tar}}$ is a mixture of simple distributions, e.g.\ a Gaussian mixture, in which case application of the transport map $T$ requires the solution of an \emph{explicit} ODE with \emph{closed-form} right-hand side. Mixture distributions are of particular applicability and interest since many methods proceed by first approximating $\mathbb{P}_{\mathrm{tar}}$ by a mixture and then sampling from that mixture (often using importance reweighting). Hence, this paper allows for the sampling step to provide a better convergence rate than $N^{-1/2}$ for all such methods.

==> section-06-SVGDwithQMCandSparseGrids.tex <==
\section{Transporting \todo{Higher Order Points} with SVGD}
\label{section:SVGDwithQMCandSparseGrids}

\todo{text}

As described in \Cref{section:ODEtransportNoPredefinedIntermediateDistributions}, SVGD realizes the transport of $\simpv$ to $\trv$ via an ODE $\dot{x}(t) = v_t(x(t))$ by choosing the velocity field in such a way that $\bP_t \to \trv$ as $t \to \infty$.
More precisely, SVGD aims at an optimal decrease of the Kullback--Leibler divergence $\dkl{\bP_t}{\trv}$, where the norm of the velocity field $v_t$ is measured in a certain \ac{RKHS} $\cH$:
\[
	v_t = \argmin_{\norm{ v }_{\cH^d}\le 1} \frac{\rd}{\rd \epsilon} \dkl {(\Id_d + \epsilon v)_{\#} \bP_t}{\trv} 
\]
Here, $\cH$ is an \ac{RKHS} corresponding to some symmetric and positive definite kernel $k\colon\bR^d\times \bR^d \to \bR$ and $\norm{ v }_{\cH^d} = (\sum_{i=1}^{d} \norm{ v_i }_\cH^2)^{1/2}$.
Surprisingly, using the theory of kernelized Stein discrepancy \citep{oates2017control, liu2016discrepancy,chwialkowski16kernel}, the above minimization problem has a closed-form solution
\begin{equation}
	\label{equ:OptimalVelocityField}
	v_t = \bE_{X\sim\bP_t} \big[k(X,\quark)\nabla\log\trd(X) + \nabla_1 k(X,\quark) \big],
\end{equation}
where $\nabla_1$ denotes the gradient with respect to the first argument.
This expected value can be approximated by \ac{MC} using samples from $\bP_t$, which suggests the following strategy:
In order to obtain $\trv$-distributed samples, start with $\simpv$-distributed samples $x_1(0),\dots,x_N(0)$ and transport them for a ``long'' time\footnote{As $\dkl{\bP_t}{\trv}$ decreases to zero, so does $\norm{ v_{t} }$ and the process converges to a stationary solution.
It is therefore sensible to stop the \ac{ODE} when $\norm{ v_{t} }$ falls below some predefined threshold.} via the approximate system of \ac{ODE}s
\begin{align}
	\notag
	\dot{x}_n(t)
	& =
	v_t^{\textup{appr}}(x_n(t)),
	\\
	\label{equ:OptimalVelocityFieldEstimated}
	v_t^{\textup{appr}}
	& =
	\frac{1}{N}\sum_{m=1}^{N} k(x_m(t),\quark)\nabla\log\trd(x_m(t)) + \nabla_1 k(x_m(t),\quark),
\end{align}
with $n=1,\dots,N$.
We will denote the final points by $x_n(\infty)$.
Naturally, \ac{MC} is not the only possible way to estimate the expected value in \eqref{equ:OptimalVelocityField} and \ac{QMC} or sparse grids might improve the approximation error, if the initial samples were chosen as a \ac{QMC} sequence or a sparse grid, respectively.
In the case of sparse grids, the approximate velocity field $v_t^{\textup{appr}}$ in \eqref{equ:OptimalVelocityFieldEstimated} needs to be replaced by a weighted average with the corresponding sparse grid weights:
\begin{align*}
	\dot{x}_n(t)
	& =
	v_t^{\textup{QMC}}(x_n(t)),
	\\
	v_t^{\textup{QMC}}
	& =
	\sum_{m=1}^{N} w_{m} \bigl( k(x_m(t),\quark)\nabla\log\trd(x_m(t)) + \nabla_1 k(x_m(t),\quark) \bigr),
\end{align*}
The advantages are two-fold.
Not only will the approximate velocity field $v_t^{\textup{appr}}$ be closer to the optimal one, also the final points $x_n(\infty)$ would represent a $\trv$-distributed \ac{QMC} sequence or sparse grid, respectively.
This reasoning would only be accurate if the flow $\Phi_t$ of the ODE \eqref{equ:OptimalVelocityFieldEstimated} were an exact transport map from $\simpv$ to $\bP_t$.
Since this will hold only approximately, these conclusions have to be drawn with great caution.
The main obstacle stems from the repulsion of the \ac{SVGD} particles and is discussed in the following section.

\todo{Also cite \citet{duncan2019stein}?}

\subsection{Repulsion within \ac{SVGD}}
It is well-known that the term $\nabla_1 k(x_m(t),\quark)$ introduces a repulsion between the points such that \ac{SVGD} tends to separate them, making them much more evenly distributed than could be expected from independent samples.
Observe how evenly the outer points in the left plot of 	\Cref{fig:TransportingMCQMCsparseGridsBySVGD} are distributed.
This has advantages and disadvantages:
On the one hand, this is not what we were aiming at.
The coupling of the \ac{ODE}s introduces a repulsion and thereby an unintended dependence of the points.
Hence, the standard versions of the law of large numbers and the central limit theorem no longer apply and it is unclear if and how the empirical mean $\frac{1}{N} \sum_{n=1}^{N} f(Y_n)$ in \Cref{MCapproximation} with $Y_n = x_n(\infty)$ converges to $\bE_{Y\sim \trv}[f(Y)]$.
On the other hand, since the points are more evenly spread, one might hope for a better coverage of the space and a super-root-$N$ convergence rate of the empirical estimate in \Cref{MCapproximation}.

While the repulsion term of \ac{SVGD} introduces the dependence of the samples in the case of MC, it might similarly impair the delicate structures of \ac{QMC} (low discrepancy) and sparse grids.



In our numerical experiments we made the following observations. In the case of MC and QMC the repulsion led to a rather structured point set, especially the outer points are evenly distributed as can be seen in \Cref{fig:TransportingMCQMCsparseGridsBySVGD}.
Consequently, the results of \ac{MC} and \ac{QMC} were almost identical.
In fact, we obtained similar results no matter which (pairwise different) points we started with.
In the case of sparse grids, however, such an effect could not be observed and the transported seemed to preserve the desired structure (\Cref{fig:TransportingMCQMCsparseGridsBySVGD}).
Since sparse grids approximate $v_t$ by a weighted average with both positive and negative weights of the points, the repulsion (and attraction!) is more difficult to comprehend in this case.

\todo{Investigate the repulsion effect in the case of quadratures with weights of both signs.
Conjecture:
particles with like-signed weights repel, and particles with opposite-signed weights attract, at least in some limiting sense.}

These questions remain important open problems for the future.
We should stress that even the \ac{MC} case, i.e.\ with initially independent samples as suggested so far for \ac{SVGD}, is not yet sufficiently analyzed, but the success of \ac{SVGD} partly justifies its wide use despite the lack of theoretical understanding.




\begin{figure}[t]
	\centering         	
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/posterior_with_SVGD_points_MC}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/posterior_with_SVGD_points_QMC}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.32\textwidth}
		\centering
		\includegraphics[width=\textwidth]{images/posterior_with_SVGD_points_sparse_grid}
	\end{subfigure}	
	\caption{Transportation of \ac{MC}, \ac{QMC}, and SG points via approximate SVGD with approximate vector field also evaluated using \ac{MC}, \ac{QMC}, and SG particles, respectively.
	\todo{MORE}}
	\label{fig:TransportingMCQMCsparseGridsBySVGD}
\end{figure}


\begin{figure}[t]
	\centering         	
	\includegraphics[width=0.6\textwidth]{images/TransportSVGDerrorPlot}
	\caption{Convergence plots for the integrand $f(y) = \exp(-\alpha y_{1}^{2})$ with $\alpha = 0.01$.
		SVGD transport from a standard normal distribution $\simpv = \cN(0,\Id_2)$ to the Gaussian distribution \todo{}.
		\todo{label the axes}}
\end{figure}





